Crop Planning using Stochastic Visual Optimization

As the world population increases and arable land decreases, it becomes vital to improve the productivity of the agricultural land available. Given the weather and soil properties, farmers need to take critical decisions such as which seed variety to plant and in what proportion, in order to maximize productivity. These decisions are irreversible and any unusual behavior of external factors, such as weather, can have catastrophic impact on the productivity of crop. A variety which is highly desirable to a farmer might be unavailable or in short supply, therefore, it is very critical to evaluate which variety or varieties are more likely to be chosen by farmers from a growing region in order to meet demand. In this paper, we present our visual analytics tool, ViSeed, showcased on the data given in Syngenta 2016 crop data challenge 1 . This tool helps to predict optimal soybean seed variety or mix of varieties in appropriate proportions which is more likely to be chosen by farmers from a growing region. It also allows to analyse solutions generated from our approach and helps in the decision making process by providing insightful visualizations

==> Sections/Criteria.tex <==
We use an expected yield based on a model using sub-region wise predictions of weather and soil conditions, standard deviation of the expected yield, and spatial cohesion as the criteria to select seed varieties. Our approach to select seed varieties involves predicting weather and soil condition attributes for each sub-region using popular recurrent neural network LSTM~(\cite{hochreiter1997long}) and then using these attributes to predict the expected yield of every sub-region. We use Random forest classifier model~(\cite{breiman2001random}) for the prediction of probability distribution of yield for every sub-region. We also tried other machine learning algorithm for classification like SVM, Gradient boosting classifier, Decision tree, but Random forest works best in terms of accuracy for our case. Further, we use an optimization method to find the combination of seed varieties in an appropriate proportion in order to maximize yield and minimize standard deviation in the predicted yield. Note, as we need probability distribution of yield as an input to optimization model rather than a single value, we use classifier instead of regression to predict yield. We also find spatial cohesion score for every solution obtained from optimization model. Solutions with high spatial cohesion scores have similar varieties in neighboring sub-regions.
